Integrating Pre-Trained Language Model with Physical Layer Communications

The burgeoning field of on-device AI communication, where devices exchange information directly through embedded foundation models, such as language models (LMs), requires robust, efficient, and generalizable communication frameworks. However, integrating these frameworks with existing wireless systems and effectively managing noise and bit errors pose significant challenges. In this work, we introduce a practical ondevice AI communication framework, integrated with physical layer (PHY) communication functions, demonstrated through its performance on a link-level simulator. Our framework incorporates end-to-end training with channel noise to enhance resilience, incorporates vector quantized variational autoencoders (VQ-VAE) for efficient and robust communication, and utilizes pre-trained encoder-decoder transformers for improved generalization capabilities. Simulations, across various communication scenarios, reveal that our framework achieves a 50% reduction in transmission size while demonstrating substantial generalization ability and noise robustness under standardized 3GPP channel models.

==> table/complexity.tex <==
\begin{tabular} {l l}
\toprule[1pt]
\textbf{Computational Complexity} &  \\
\midrule
% \emph{\textbf{Channel En/Decoder}} \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2}
FLOP [GFLOPSs] & \tcyan{XXX} \\ 
Memory & \tcyan{XXX} \\
Latency [ms] & \tcyan{XXX} \\
Model size [MB] & \tcyan{XXX} \\
\bottomrule[1pt]
\end{tabular}


==> table/impact_pretrain.tex <==
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\begin{tabularx}{1\linewidth}{c | c c | c c }
\toprule[1.5pt]
\textit{\textbf{Pre-Training}} & \textit{\textbf{Fine-Tuning}} & \textit{\textbf{Dataset}} & \multirow{2}{*}{\textit{\textbf{BLEU}}$\uparrow$} & \multirow{2}{*}{\textit{\textbf{SBERT}}$\uparrow$}  \\
(\texttt{BART}) & on &  for Eval. &   &  \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
\joohan{\xmark} & Europarl & Europarl & 0.0071 & 0.2235  \\
\cmark & Europarl & Europarl & 0.9823 & 0.9952   \\
\xmark & Europarl & Flickr & 0 & -0.0228  \\
\cmark & Europarl & Flickr & 0.9825 & 0.9998   \\
\bottomrule[1.5pt]
\end{tabularx}

==> table/parameter_train.tex <==
\begin{tabular} {l l}
\toprule[1pt]
\textbf{Parameter} & \textbf{Value} \\
% \midrule
% \emph{\textbf{Train}} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2}
Optimizer & Adam \\
\# of epochs & 3 \\
Learning rate (LR) & 5e-5 \\
LR scheduler type & linear \\
Batch size & 4 \\
\midrule
% \emph{\textbf{Dataset}} \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2}
\textbf{Dataset} & \textbf{\# of Training (Validation) Data} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-2} 
Europarl \cite{koehn-2005-europarl}  & $66125$ $(7347)$ \\ 
% STS Benchmark \cite{46231} & $2063$ $(404)$ \\ 
Flickr30k \cite{Young2014FromID} & $1000$ (sampled for testset) \\ 
\bottomrule[1pt]
\end{tabular}

